Emergent Communication with Attention

To develop computational agents that better communicate using their own emergent language, we endow the agents with an ability to focus their attention on particular concepts in the environment. Humans often understand an object or scene as a composite of concepts and those concepts are further mapped onto words. We implement this intuition as cross-modal attention mechanisms in Speaker and Listener agents in a referential game and show attention leads to more compositional and interpretable emergent language. We also demonstrate how attention aids in understanding the learned communication protocol by investigating the attention weights associated with each message symbol and the alignment of attention weights between Speaker and Listener agents. Overall, our results suggest that attention is a promising mechanism for developing more human-like emergent language.

==> sections/figures/additional_results.tex <==
\begin{figure*}[t]
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (8, 2): \TrainAcc}]{\label{fig:add-onehot_8_2-train}\includegraphics[width=\figWidth]{data/main_results/onehot_8_2-train.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (8, 2): \GenAcc}]{\label{fig:add-onehot_8_2-gen}\includegraphics[width=\figWidth]{data/main_results/onehot_8_2-eval.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (8, 2): \TopSim}]{\label{fig:add-onehot_8_2-topsim}\includegraphics[width=\figWidth]{data/main_results/onehot_8_2-topsim.png}}
\end{minipage}\par\medskip % ============================================
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (4, 4): \TrainAcc}]{\label{fig:add-onehot_4_4-train}\includegraphics[width=\figWidth]{data/appendix_results/onehot_4_4-train.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (4, 4): \GenAcc}]{\label{fig:add-onehot_4_4-gen}\includegraphics[width=\figWidth]{data/appendix_results/onehot_4_4-eval.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (4, 4): \TopSim}]{\label{fig:add-onehot_4_4-topsim}\includegraphics[width=\figWidth]{data/appendix_results/onehot_4_4-topsim.png}}
\end{minipage}\par\medskip % ============================================
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (16, 2): \TrainAcc}]{\label{fig:add-onehot_16_2-train}\includegraphics[width=\figWidth]{data/appendix_results/onehot_16_2-train.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (16, 2): \GenAcc}]{\label{fig:add-onehot_16_2-gen}\includegraphics[width=\figWidth]{data/appendix_results/onehot_16_2-eval.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot (16, 2): \TopSim}]{\label{fig:add-onehot_16_2-topsim}\includegraphics[width=\figWidth]{data/appendix_results/onehot_16_2-topsim.png}}
\end{minipage}\par\medskip % ============================================
\caption{The results of the one-hot game with different configurations. The color of the boxes indicates the base architecture of the agents (LSTM or Transformer) and the x-axis labels indicates whether \Speaker and \Listener use attention.}
\label{fig:add-results}
\end{figure*}


==> sections/figures/another_baseline.tex <==
\begin{figure*}[ht]
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot: \TrainAcc}]{\label{fig:concat-onehot-train}\includegraphics[width=\figWidth]{data/appendix_results/onehot_8_2-concat-train.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot: \GenAcc}]{\label{fig:concat-onehot-gen}\includegraphics[width=\figWidth]{data/appendix_results/onehot_8_2-concat-gen.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot: \TopSim}]{\label{fig:concat-onehot-topsim}\includegraphics[width=\figWidth]{data/appendix_results/onehot_8_2-concat-topsim.png}}
\end{minipage}\par\medskip % ============================================
\caption{The comparison of different types of baseline object encoders.}
\label{fig:concat-results}
\end{figure*}


==> sections/figures/architecture.tex <==
\begin{figure*}[ht]
% ============================================
\begin{minipage}{.5\linewidth}
\centering
\subfloat[LSTM]{\label{fig:arch-lstm}\includegraphics[width=5.2cm]{data/attention_agents/LSTM.jpeg}}
\end{minipage}\hfill
% ======
\begin{minipage}{.5\linewidth}
\centering
\subfloat[Transformer]{\label{fig:arch-transformer}\includegraphics[width=5.2cm]{data/attention_agents/Transformer.jpeg}}
\end{minipage}%
% ============================================
\caption{The architecture of the LSTM and Transformer decoders used in this paper.}
\label{fig:arch}
\end{figure*}


==> sections/figures/attention_distribution.tex <==
\begin{figure*}[t]
% ======
\begin{minipage}{.25\linewidth}
\centering
\subfloat[\scriptsize{\Attn-\NoAttn: S}]{\label{fig:attention-distribution:a}\includegraphics[width=3.5cm]{data/onehot_attention_distributions/attn_S.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.25\linewidth}
\centering
\subfloat[\scriptsize{\NoAttn-\Attn: L}]{\label{fig:attention-distribution:b}\includegraphics[width=3.5cm]{data/onehot_attention_distributions/attn_L.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.25\linewidth}
\centering
\subfloat[\scriptsize{\Attn-\Attn: S}]{\label{fig:attention-distribution:c}\includegraphics[width=3.5cm]{data/onehot_attention_distributions/attn_attn_S.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.25\linewidth}
\centering
\subfloat[\scriptsize{\Attn-\Attn: L}]{\label{fig:attention-distribution:d}\includegraphics[width=3.5cm]{data/onehot_attention_distributions/attn_attn_L.png}}
\end{minipage}
% ======
\caption{The distribution of attention weights from Transformer agents in the one-hot game.}
\label{fig:attention-distribution}
\vspace{-3mm}
\end{figure*}


==> sections/figures/multi_head.tex <==


\begin{figure*}[ht]
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot: \TrainAcc}]{\label{fig:mh-onehot-train}\includegraphics[width=\figWidth]{data/appendix_results/onehot_8_2-MH-train.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot: \GenAcc}]{\label{fig:mh-onehot-gen}\includegraphics[width=\figWidth]{data/appendix_results/onehot_8_2-MH-gen.png}}
\end{minipage}\hfill%
% ======
\begin{minipage}{.33\linewidth}
\centering
\subfloat[\small{One-hot: \TopSim}]{\label{fig:mh-onehot-topsim}\includegraphics[width=\figWidth]{data/appendix_results/onehot_8_2-MH-topsim.png}}
\end{minipage}\par\medskip % ============================================
\caption{The comparison of different numbers of heads in the source-target attention of the Transformer Speaker. Listener is the non-attention Transformer model.}
\label{fig:mutli-head-results}
\end{figure*}


==> sections/memo.tex <==
On the mapping between concepts and words:~\cite{sperber_wilson_wilson_sperber_2012}


==> sections/reproducibility_statement.tex <==
\section*{Reproducibility Statement}
The experiments described in this paper are ensured to be reproducible in the following ways:

\begin{itemize}
  \item We describe the task setup and models in \cref{sec:experimental_framework} together with more specific descriptions of each task in \cref{sec:exp-setup}. The additional details and hyperparameters to reproduce the results are given in \cref{appendix:experimental_setup}.
  \item The artifacts used in the experiments (the Fashion-MNIST dataset and pretrained ConvNet encoder in \cref{subsec:fashion-mnist}) are all publicly available.
  \item The source code will be released upon acceptance.
\end{itemize}


==> sections/tables/results.tex <==
 \begin{table}[t]
    \small
    \setlength\tabcolsep{3pt}
    \centering
  \begin{tabular}{lllll|lll} \toprule
                      & \multicolumn{4}{c}{One-hot}                                                  & \multicolumn{3}{c}{Fashion-MNIST} \\
                      & \multicolumn{1}{c}{\Acc$\uparrow$}                 & \multicolumn{1}{c}{\TopSim$\uparrow$}             &  \multicolumn{1}{c}{\PosDis$\uparrow$}              & \multicolumn{1}{c}{\BosDis$\uparrow$}             &  \multicolumn{1}{c}{\Acc$\uparrow$}             &   \multicolumn{1}{c}{\TopSim$\uparrow$}          & \multicolumn{1}{c}{\BosDis$\uparrow$}          \\ \midrule
  \NoAttn-\NoAttn &   89.4$\pm$7.4                  &   55.1$\pm$6.4                 &   12.9$\pm$9.3                 &   49.3$\pm$8.4                 &  45.6$\pm$1.8                &   29.6$\pm$1.7                 & 20.0$\pm$3.9       \\ \midrule
  \Attn-\NoAttn   &   \textbf{95.9$\pm$5.3$^{*}$}   &   68.8$\pm$7.7$^{*}$           &   39.3$\pm$19.5$^{*}$          &   54.7$\pm$6.8$^{*}$           &  52.1$\pm$6.8$^{*}$          &   \textbf{51.8$\pm$6.1$^{*}$}  & 29.5$\pm$5.3$^{*}$ \\
  \NoAttn-\Attn   &   93.6$\pm$4.4$^{*}$            &   58.2$\pm$4.8                 &   21.4$\pm$12.0$^{*}$          &   \textbf{67.5$\pm$11.5$^{*}$} &  44.3$\pm$4.7                &   39.9$\pm$6.0$^{*}$           & 24.3$\pm$6.8       \\
  \Attn-\Attn     &   \textbf{95.9$\pm$4.2$^{*}$}   &   \textbf{73.5$\pm$12.0$^{*}$} &   \textbf{53.5$\pm$25.2$^{*}$} &  62.6$\pm$12.2$^{*}$           &  \textbf{54.0$\pm$4.0$^{*}$} &   51.1$\pm$3.6$^{*}$           & \textbf{31.9$\pm$8.6$^{*}$} \\
  \bottomrule
  \end{tabular}
 \caption{The results of the referential game. The leftmost column indicates the architectures of \Speaker-\Listener. The scores show the average and standard deviations of 20 different runs for the One-hot game and 10 runs for the Fashion-MNIST game. The highest average scores in each column are boldfaced. $*$ indicates scores with statistically significantly improvement ($p < 0.05$ in Welch's t-test) over \NoAttn-\NoAttn.}
 \label{table:results}
\end{table}

